FIGROTD: A Friendly-to-Handle Dataset for Image Guided Retrieval with Optional Text

Image-Guided Retrieval with Optional Text (IGROT) unifies visual retrieval (without text) and composed retrieval (with text). Despite its relevance in applications like Google Image and Bing, progress has been limited by the lack of an accessible benchmark and methods that balance performance across subtasks. Large-scale datasets such as MagicLens are comprehensive but computationally prohibitive, while existing models often favor either visual or compositional queries. We introduce FIGROTD, a lightweight yet high-quality IGROT dataset with 16,474 training triplets and 1,262 test triplets across CIR, SBIR, and CSTBIR. To reduce redundancy, we propose the Variance Guided Feature Mask (VaGFeM), which selectively enhances discriminative dimensions based on variance statistics. We further adopt a dual-loss design (InfoNCE + Triplet) to improve compositional reasoning. Trained on FIGROTD, VaGFeM achieves competitive results on nine benchmarks, reaching 34.8 mAP@10 on CIRCO and 75.7 mAP@200 on Sketchy, outperforming stronger baselines despite fewer triplets.

==> section/table/data_comparison.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l c | l l r r | l l r r}
\toprule
\textbf{Dataset} & \textbf{Public} & \multicolumn{4}{c|}{\textbf{Reference-Target Image Pair}} & \multicolumn{4}{c}{\textbf{Modification Text Generation}} \\
 & & \textbf{Type} & \textbf{Source} & \textbf{\# Pairs} & \textbf{\# Entities} & \textbf{LLM} & \textbf{LLM input} & \textbf{\# Text} & \textbf{\# Text/Pair} \\
\midrule
LaSCo& ✓ & image & VQAv2& 360K & 82K & GPT-3& question-answer & 360K & 1 \\
VDG& ✓ & image & NLVR2~\href{https://arxiv.org/abs/xxxx}{}, COCO& 467K & 183K & Vision-LLaMA2 & image pair & 523K & 1.12 \\
WebCoVR& ✓ & video & WebVid2M& 1.6M & 131K & Custom LLM & caption & 1.6M & 1 \\
CC-CoIR& ✓ & image & CC3M& 3.3M & 357K & Custom LLM & caption & 3.3M & 1 \\
SynthTriplets& ✓ & synth. image & SD~\href{https://arxiv.org/abs/xxxx}{}, IP2P& 18.8M & 37.6M & OPT-6.7B& - & 18.8M & 1 \\
MagicLens& ✓ & image & Web crawled & 36.5M & - & PaLM& image metadata & 36.5M & 1 \\
\rowcolor{blue!5}
MTCIR (Ours) & ✓ & image & LLaVA-558k& 3.4M & 423K & Sonnet 3& synth. caption & 17.7M & 5.18 \\
\bottomrule
\end{tabular}}
\caption{Comparison of Composed Image Retrieval datasets and their text generation approaches.}
\end{table*}


==> section/table/lambda_result.tex <==
\begin{table}[!hbt]
\centering
\caption{Impact of the parameter $\alpha$ on the result}
% \vspace{0.1in}
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{$\lambda$} & \multicolumn{4}{c}{\textbf{VQA-RAD}}      \\ \cmidrule{2-5} 
                          & Open  & Close & Avg.  & Run Time \\ \midrule
0.1   & 55.9  & 73.9  & 64.9  & 1h       \\
0.3   & 66    & 79.04 & 72.52 & 1h4'     \\
0.5   & 55.52 & 73.16 & 64.37 & 1h17'    \\ \bottomrule
\end{tabular}
\label{tab:alpha}
\end{table}

==> section/table/param_result.tex <==
\begin{table}[!hbt]
% \centering
% \vspace{0.1in}
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{cc}
\begin{minipage}{.5\linewidth}
    \caption{Impact of the parameter $\alpha$ on the result}
    \centering
    \begin{tabular}{l|cc|cc|c}
    \toprule
    \multirow{2}{*}{$\alpha$} & \multicolumn{2}{c|}{\textbf{FashionIQ}}   & \multicolumn{2}{c|}{\textbf{TUBerlin}} & \textbf{PatCom}    \\ \cmidrule{2-6} 
        & R@10  & R@50 & mAP  & P@100 & AVG mAP \\ \midrule
    0.1   & 55.9  & 73.9  & 64.9  & a & a      \\
    0.3   & 66    & 79.04 & 72.52 & a & a     \\
    0.5   & 55.52 & 73.16 & 64.37 & a & a   \\ \bottomrule
    \end{tabular}
\end{minipage}% 

\begin{minipage}{.5\linewidth}
    \caption{Impact of the parameter $\lambda$ on the result}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{$\lambda$} & \multicolumn{4}{c}{\textbf{VQA-RAD}}      \\ \cmidrule{2-5} 
                              & Open  & Close & Avg.  & Run Time \\ \midrule
    0.1   & 55.9  & 73.9  & 64.9  & 1h       \\
    0.3   & 66    & 79.04 & 72.52 & 1h4'     \\
    0.5   & 55.52 & 73.16 & 64.37 & 1h17'    \\ \bottomrule
    \end{tabular}
\end{minipage}% 
\end{tabular}


\label{tab:param}
\end{table}

==> section/table/patterncom_result.tex <==
% \vspace{-0.1in}
% \begin{wrapfigure}{r}{0.4\textwidth}
%     \centering % Centers the figure within the wrapfigure
%     \vspace{-0.2in}
    \begin{table}[!hbt]
    \centering
        \begin{tabular}{lccccccc}
    \hline Method & Color & Context & Density & Existence & Quantity & Shape & AVG \\
    \hline WEICOM $_{CLIP}$ & 46.74 & 20.97 & 22.07 & 12.07 & 20.96 & 26.22 & 24.83 \\
    \hline WEICOM $_{RemoteCLIP}$ & 41.04 & 31.59 & 41.56 & 14.79 & 20.79 & 31.24 & 30.19 \\
    \hline CLIP ViT-L/14 & 34.31 & 25.58 & 38.35 & 36.85 & 13.24 & 38.05 & 31.06 \\ 
    \hline BLIP & 31.82 & 34.46 & 19.11 & 23.53 & 11.17 & 29.08 & 24.86 \\
    \hline
\end{tabular}
    \caption{Results of Remote Sensing Dataset }
        \label{tab:placeholder}
    \end{table}
%     \vspace{-0.1in }
%     \label{fig:patterncom_result}
% \end{wrapfigure}

==> section/table/triplet_loss_result.tex <==
\begin{table}[!hbt]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccc}
\hline 
Method & \makecell{FIQ\\(R@10)} & \makecell{CIRR\\(R@10)} & \makecell{CIRCO\\(mAP@10)} & \makecell{PatternCom\\(mAP)} & \makecell{Sketchy\\(mAP@200)} & \makecell{TUBerlin\\(mAP)} & \makecell{QuickDraw\\(mAP)} & \makecell{PKU\\(mAP)} & AVG \\
\hline  
TransAgg & x & x & x & x & x & x & x & x & x \\
\hline 
TransAgg$_\text{Triplet}$ & x & x & x & x & x & x & x & x & x \\
\hline 
VaGFeM & 26.35 & 76.57 & 32.42 & 19.65 & 74.86 & 62.04 & 24.07 & 24.50 & 42.56 \\ 
\hline 
VaGFeM$_\text{Triplet}$ & 29.26 & 76.38 & 33.97 & 25.00 & 75.03 & 60.79 & 22.53 & 22.76 & 43.22 \\
\hline
\end{tabular}
}
\caption{Results of Triplet Loss}
\label{tab:placeholder}
\end{table}
